Average Token Delay: A Latency Metric for Simultaneous Translation

Simultaneous translation is a task in which translation begins before the speaker has finished speaking. In its evaluation, we have to consider the latency of the translation in addition to the quality. The latency is preferably as small as possible for users to comprehend what the speaker says with a small delay. Existing latency metrics focus on when the translation starts but do not consider adequately when the translation ends. This means such metrics do not penalize the latency caused by a long translation output, which actually delays users' comprehension. In this work, we propose a novel latency evaluation metric called Average Token Delay (ATD) that focuses on the end timings of partial translations in simultaneous translation. We discuss the advantage of ATD using simulated examples and also investigate the differences between ATD and Average Lagging with simultaneous translation experiments.

==> x_experiment.tex <==
%\section{Experimental Setup}
%below sentences commented out is from IWSLT

% We conducted experiments on English-to-German (En-De) and English-to-Japanese (En-Ja) simultaneous translation to compare the proposed method with the baselines in the quality-latency trade-off.

% \subsection{Dataset and Preprocessing}
% In En-De translation, we used WMT 2014 training set (4.5 M sentence pairs) for pre-training and IWSLT 2017 training set (206 K sentence pairs) for fine-tuning. 
% We used IWSLT dev2010, tst2010, tst2011 and tst2012 (5,589 sentence pairs in total) for the development dataset.
% We used 1,080 sentence pairs from IWSLT tst2015 for the evaluation.

% In En-Ja translation, we used WMT 2020 (17.9 M sentence pairs) for pre-training and IWSLT 2017 (223 K sentence pairs) for fine-tuning dataset. 
% We used IWSLT dev2010, tst2011, tst2012, and tst2013 (5,312 sentence pairs in total) for development dataset. 
% We used 1,442 sentence pairs from IWSLT dev2021 for the evaluation.

% Prefix translation pairs are collected only from the IWSLT dataset.
% We tokenized Japanese sentences using MeCab \cite{kudo2005}.
% English and German sentences were tokenized using \texttt{tokenizer.perl} in Moses \cite{koehn-etal-2007-moses}. 
% We prepared a shared subword vocabulary with 16 K entries based on Byte Pair Encoding (BPE) \cite{sennrich-etal-2016-neural} for each language pair.


% \subsection{Model Settings}

% We mainly compared the following four methods in the experiments:

% \paragraph{Prefix Alignment}
% % We can adjust the latency by the proposed method using a threshold offset for the boundary prediction.
% The proposed method has a hyperparameter to adjust latency, the threshold of boundary probability output by the boundary predictor.
% We used 0.5 as the default value for the binary classification and tried the following values for further investigation: [0.1, 0.15,..., 0.95], [0.99, 0.991, 0.992,..., 0.999], and [0.9991, 0.9992,..., 0.9999].
% We also compared a one look-ahead boundary predictor that took one future word as the input at the cost of the delay in one word (\texttt{PA-1}), in addition to a standard (no look-ahead) boundary predictor (\texttt{PA-0}).
% %We compared this model with and without future 1 word for the boundary prediction.

% \paragraph{Meaningful Unit}
% We used the same boundary probability thresholds as in PA.
% We implemented the refined version of MU-based method to translate with low latency following \cite{zhang-etal-2020-learning-adaptive},
% but did not apply the removal of monotonic translation examples following \newcite{kano-etal-2021-simultaneous}.
% %\footnote{Originally, \newcite{zhang-etal-2020-learning-adaptive} removed monotonic translations with the scores lower than the full-sentence translation from their fine-tuning data. 
% %However, monotonic translations rarely have higher scores than full-sentence translations, so we 
% %Therefore, the detailed implementation followed \citet{kano-etal-2021-simultaneous}.}.
% We also compared one look-ahead (\texttt{MU-1}) and no look-ahead (\texttt{MU-0}) boundary predictors.

% \paragraph{Incremental Constitutent Label Prediction (\texttt{ICLP})}
% Following \citet{kano-etal-2021-simultaneous}, we used a one look-ahead label predictor.
% We segmented the input sequence based on their rules with the predicted labels \texttt{VP} and \texttt{S}. The minimum segment length adjusts latency. The range is  [1, 2, 3, ..., 29].

% \paragraph{\texttt{Wait-k}}
% We tried [2, 4, 6, ..., 30] for the hyperparameter \textit{k}.

% \paragraph{NMT Settings}
% All the NMT models were based on Transformer-base \cite{vaswani-2017} implemented with fairseq \cite{ott-etal-2019-fairseq}. 
% Their hyperparameter settings basically followed the official baseline for IWSLT 2021\footnote{\url{https://github.com/pytorch/fairseq/blob/master/examples/simultaneous_translation/docs/enja-waitk.md}, \url{https://github.com/pytorch/fairseq/issues/346}}, for both pre-training and fine-tuning.
% The models were saved on checkpoints in every 5,000 updates for pre-training and every 200 updates for fine-tuning. 
% We applied early stopping with the patience for four checkpoints, based on the loss on the development set. 
% %Other hyperparameters were the same for pre-training and fine-tuning. 
% We set the learning rate to 0.0007, minibatch size to 4,096 with the parameter update frequency of 4.
% %The maximum number of tokens for a minibatch was 4096, and weights were updated every 4 mini batches. 
% We applied a chunk-based beam search for the methods other than wait-k,
% in which the low-scored hypotheses out of the specified beam size were eliminated at the end of the chunk.
% We used greedy-decoding for wait-k, due to the nature of its model.

% \paragraph{Boundary Predictor}
% The boundary predictors for the chunk-based methods were implemented similarly using BERT \cite{devlin-etal-2019-bert}
% with a pre-trained model \texttt{bert-base-uncased} and the corresponding subword tokenizer from Huggingface transformers \cite{wolf-etal-2020-transformers}.
% We set the learning rate to 5e-5 and the batch size to 512 instances.
% The models were saved at every epoch, and we applied early stopping with patience for three epochs based on the loss on the development set.

% \subsection{Evaluation Metrics}
% We used BLEU \cite{papineni-etal-2002-bleu} and Average Lagging (AL) \cite{ma-etal-2019-stacl} for our quality and latency evaluation metrics.
% They were calculated using SimulEval \cite{ma-etal-2020-simuleval} and drawn in scatterplots to show the quality-latency trade-off.
% % to evaluate quality-latency trade-off of the models.
% % BLEU \cite{papineni-etal-2002-bleu} was used to evaluate the quality. 
% % Latency was evaluated with Average Lagging (AL) which follows the equation bellow.

% % \begin{equation}
% % AL_g(X, Y) = \frac{1}{\tau_g(|X|)}\sum_{t = 1}^{\tau_g(|X|)}g(t) - \frac{t-1}{\gamma}.
% % \end{equation}

% % $g(t)$ is a monotonic non-decreasing function and means the number of read source tokens to output the $t$ th target token. 
% % $\tau_g(|X|)$ is the decoding step when the final source token has been read. $\gamma$ is defined as $|Y|/|X|$.


